Worst-Case Sensitivity of DC Optimal Power Flow Problems

In this paper we consider the problem of analyzing the effect a change in the load vector can have on the optimal power generation in a DC power flow model. The methodology is based upon the recently introduced concept of the $\mathcal{OPF}$ operator. It is shown that for general network topologies computing the worst-case sensitivities is computationally intractable. However, we show that certain problems involving the $\mathcal{OPF}$ operator can be equivalently converted to a graphical discrete optimization problem. Using the discrete formulation, we provide a decomposition algorithm that reduces the computational cost of computing the worst-case sensitivity. A 27-bus numerical example is used to illustrate our results.

==> Sensitivity for arXiv/decomp.tex <==
\floatstyle{spaceruled}% Select new float style
\restylefloat{algorithm}% Apply spaceruled float style to algorithm
\begin{algorithm} % enter the algorithm environment
\caption{Decomposition of the computation of $C_{i\leftarrow j}^{\mathrm{wc}}$.}
\label{alg2}
\begin{algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\algorithmiccompute}{\textbf{compute }}
\newcommand{\CALL}{\STATE \algorithmiccall }
\newcommand{\algorithmiccall}{\textbf{call }}
\newcommand{\COMPUTE}{\STATE \algorithmiccompute }
    \REQUIRE $\B$, $\CM$, $i\in[\nG]$, $j\in[\nL]$, $\Graph(\VertexG\cup\VertexL,\Edge)$
    \ENSURE $C_{i\leftarrow j}^{\mathrm{wc}}$
    \FOR{$e=(u,v)$ in $\Edge^{\rm bri}$}
    	\IF{$u,v\not\in\VertexG$ and $v_i\Leftrightarrow v_{j+\nG}$ in $\Graph(\Vertex,\Edge\setminus\{e\})$}
		\STATE $e$ partitions $\Graph$ into $\Graph_1$ and $\Graph_2$ (assume $v_i, v_{j+\nG}$ are both in $\Graph_1$)
		\IF{$\Graph_2$ contains any vertex in $\VertexG$}
			\STATE Replace $\Graph_2$ by a single generator
		\ELSE
			\STATE Replace $\Graph_2$ by a single load
		\ENDIF
	\ENDIF
    \ENDFOR
    \STATE Find a shortest path connecting $v_i$ and $v_{j+\nG}$
    \STATE Get $\{\Graph_{l}\}_{l=1}^m$ and add $p_l$, $q_l$ to subgraphs
    \FOR{$l=0$ to $m-1$}
    	\CALL subroutine to compute $C_{p_l\leftarrow q_{l+1}}^{\mathrm{wc}}$
    \ENDFOR
    \STATE $C_{i\leftarrow j}^{\mathrm{wc}}\leftarrow \prod_{l=0}^{m-1} C_{u_l\leftarrow v_{l+1}}^{\mathrm{wc}}$
    \RETURN $C_{i\leftarrow j}^{\mathrm{wc}}$
\end{algorithmic}
\end{algorithm}

In this subsection, we provide an algorithm which can decompose the computation  of the worst-case SISO sensitivity of generator $i$ with respect to load $j$ into  sub-problems  involving computations on smaller graphs when $\Graph$ has bridges. 
Recall that the worst-case SISO sensitivity problem formulated in \eqref{eq:wcsen} is non convex and thereby difficult to solve for large networks. 
This algorithm aims to reduce the computational complexity by breaking the large-scale computation down into independent smaller tasks, which are usually much easier than the original problem and can be processed in parallel.





Here a bridge is an edge in $\Edge$ whose deletion disconnects the graph.
Define $\Edge^{\rm bri}$ as the set of bridges in $\Edge$.
In a not necessarily connected graph $\Graph'$, we say $v_i\Leftrightarrow v_{j+\nG}$ if there exists a path between nodes $v_i$ and $v_{j+\nG}$ .

In the first step, for any bridge $e=(u,v)\in\Edge^{\rm bri}$ that partitions $\Graph$ into $\Graph_1$ and $\Graph_2$,
 if $v_i\Leftrightarrow v_{j+\nG}$ after $e$ is deleted, then without loss of generality we assume both $v_i$ and $v_{j+\nG}$ are in $\Graph_1$.
 In this case we can replace the whole of $\Graph_2$ by a single bus. The rule is if $\Graph_2$ contains only load buses then it will be replaced by a single load, else it is replaced by a single generator.
 
 In the second step, we find a shortest path (in terms of the number of edges along the path) connecting $v_i$ and $v_{j+\nG}$,
 and the bridges along the path will partition the graph into subgraphs $\{\Graph_l(\Vertex_l,\Edge_l)\}_{l=1}^m$.
Assume the indices are assigned such that $\Graph_{l-1}$ is always closer to $v_i$ than $\Graph_l$. 
At the location of each bridge 
connecting $\Graph_{l-1}$ and $\Graph_l$, 
we add a single load $q_{l-1}$ to $\Graph_{l-1}$ and a single generator $p_{l-1}$ to $\Graph_l$, as shown in Figure \ref{Fig:Alg}.
For notational consistency,
we refer to $i$ as generator $p_0$ and $j$ as load $q_m$.
Then the computation of $C_{i\leftarrow j}^{\mathrm{wc}}$ can be composed as $\prod_{l=0}^{m-1} C_{p_l\leftarrow q_{l+1}}^{\mathrm{wc}}$,
where each $C_{p_l\leftarrow q_{l+1}}^{\mathrm{wc}}$ only depends on computing the sensitivity for smaller graphs.
This procedure is summarized as Algorithm \ref{alg2}.


\begin{figure*}[ht]
\vspace*{0.2cm}
\centering
\includegraphics[width=1.7\columnwidth]{./Figs/alg.png}
\caption{Algorithm to decompose the worst-case SISO sensitivity of generator $i$ with respect to load $j$ into computation involving smaller graphs. Step1: Replace the off-path subgraphs by a single node. 
Step 2: Partition the on-path subgraphs and complement each subgraph by adding a pair of generator/load. }
\label{Fig:Alg}
\end{figure*}












==> Sensitivity for arXiv/info.tex <==
% Packages and macros go here
\usepackage{lipsum}
\usepackage{epstopdf}
%\usepackage{booktabs} % For formal tables
\usepackage{amsfonts}
\usepackage{mathrsfs} 
\usepackage{amsmath} 
\usepackage{psfrag} 
%\usepackage{multirow} 
%\usepackage{arydshln}
\usepackage{enumerate}
%\usepackage{bbm}
%\usepackage{graphicx}
\usepackage{mathtools}
%\usepackage{color}
%\usepackage{setspace}
%\usepackage{float}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{scalerel}
\usepackage{comment}
\usepackage{gensymb}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{accents}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%\newtheorem{assumption}{Assumption}
%\newcolumntype{Y}{>{\centering\arraybackslash}X}


% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}


% macros
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\mind}{\min.}
\DeclareMathOperator{\sgn}{sgn}

%\newcommand{\st}{\text{subject to}}
\newcommand{\suchthat}{\text{such that}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Sspace}{\mathbb{S}^+}
\newcommand{\Zset}{\mathbb{Z}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\co}{\mathsf c}
\newcommand{\rank}{{\rm rank}}
\newcommand{\inte}{{\mathrm{int}}}
\newcommand{\clos}{{\mathrm{clos}}}
\newcommand{\base}{{\bf{e}}}
\newcommand{\eye}{\mathbf{I}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\const}{{\rm constant}}
\newcommand{\Ind}{\mathbbm{1}}
\newcommand{\opt}{{\rm opt}}
\newcommand{\fea}{{\rm fea}}
\newcommand{\diff}{\mathrm{d}}

\newcommand{\alphavec}{\boldsymbol{\alpha}}
\newcommand{\betavec}{\boldsymbol{\beta}}

\newcommand{\Graph}{\mathcal{G}}
\newcommand{\Graphnew}{\mathcal{G}_{\rm new}}
\newcommand{\Vertex}{\mathcal{V}}
\newcommand{\VertexG}{\mathcal{V}_{\rm{G}}}
\newcommand{\VertexL}{\mathcal{V}_{\rm{L}}}
\newcommand{\Edge}{\mathcal{E}}
\newcommand{\EdgeI}{\mathcal{E}^{\rm I}}
\newcommand{\EdgeII}{\mathcal{E}^{\rm II}}

\newcommand{\RVertex}{\mathcal{R}}

\newcommand{\nG}{N_{\rm{G}}}
\newcommand{\nL}{N_{\rm{L}}}
\newcommand{\nGL}{N}
\newcommand{\nE}{E}

\newcommand{\CM}{\mathbf{C}}
\newcommand{\B}{\mathbf{B}}

\newcommand{\sgen}{\mathbf{s}^g}
\newcommand{\sgens}{\mathbf{s}_*^g}
\newcommand{\sload}{\mathbf{s}^l}
\newcommand{\sloads}{\mathbf{s}_*^l}
\newcommand{\sloadss}{\mathbf{s}_{**}^l}
\newcommand{\pf}{\mathbf{p}}
\newcommand{\genllim}{\underline{\mathbf{s}}^g}
\newcommand{\genulim}{\overline{\mathbf{s}}^g}

\newcommand{\ang}{\boldsymbol{\theta}}
\newcommand{\angs}{\boldsymbol{\theta}_*}
\newcommand{\f}{{\bf f}}
\newcommand{\fs}{{\bf f}_*}
\newcommand{\fss}{{\bf f}_{**}}
\newcommand{\M}{{\bf M}}
\newcommand{\RelationMat}{{\bf H}}
\newcommand{\subRelationMat}{{\bf H}_1}
\newcommand{\bigMat}{{\bf R}}
\newcommand{\pflow}{{\bf p}}
\newcommand{\pflows}{{\bf p}_*}
\newcommand{\taueq}{\boldsymbol{\tau}}
\newcommand{\mup}{\boldsymbol{\mu}_+}
\newcommand{\mum}{\boldsymbol{\mu}_-}
\newcommand{\mupm}{\boldsymbol{\mu}}
\newcommand{\lambdap}{\boldsymbol{\lambda}_+}
\newcommand{\lambdam}{\boldsymbol{\lambda}_-}
\newcommand{\lambdapm}{\boldsymbol{\lambda}}
\newcommand{\set}{\Omega}
\newcommand{\setbad}{\Omega_{\rm bad}}
\newcommand{\setf}{\Omega_{\f}}
\newcommand{\setsl}{\Omega_{\sload}}
\newcommand{\setsg}{\Omega_{\sgen}}
\newcommand{\setpara}{\Omega_{\para}}
\newcommand{\setall}{\Omega}
\newcommand{\setallr}{\tilde{\Omega}}
\newcommand{\para}{{\boldsymbol{\xi}}}
\newcommand{\paras}{{\boldsymbol{\xi}}_*}
\newcommand{\parass}{{\boldsymbol{\xi}}_{**}}
\newcommand{\setslr}{\widetilde{\Omega}_{\sload}}
\newcommand{\setsgr}{\widetilde{\Omega}_{\sgen}}
\newcommand{\setparar}{\widetilde{\Omega}_{\para}}

\newcommand{\lbold}{\boldsymbol{\lambda}}
\newcommand{\nubold}{\boldsymbol{\nu}}

\newcommand{\setR}{\mathcal{R}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setT}{\mathcal{T}}
\newcommand{\setQ}{\mathcal{Q}}

\newcommand{\OPF}{\mathcal{OPF}}

\newcommand{\JM}{\mathbf{J}}
\newcommand{\Jwc}{\mathbf{J}^{\rm w}}
\newcommand{\Jsum}{{\boldsymbol \chi}}
\newcommand{\setSgen}{\setS_{\rm G}}
\newcommand{\setSbra}{\setS_{\rm B}}

\newcommand{\Cut}{\mathcal{C}}
\newcommand{\qvec}{{\bf q}}
\newcommand{\tqvec}{\tilde{{\bf q}}}

\newcommand{\dpnoise}{Y}
\newcommand{\mech}{\mathcal{M}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Lap}{\mathscr{L}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\data}{\mathbf{d}}
\newcommand{\dpnoises}{{\bf{Y}}}

\newcommand{\dD}{\mathrm{d}}

% For appendix
\newcommand{\loosegen}{\aleph}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\X}{{\bf X}}
\newcommand{\Y}{{\bf Y}}
\newcommand{\ytilde}{\tilde{\bf y}}
\newcommand{\yreduce}{\underline{\bf y}}
\newcommand{\ytildereduce}{\underline{\tilde{\bf y}}}
\newcommand{\z}{{\bf z}}
\newcommand{\Aeq}{{\bf A}_{\rm{eq}}}
\newcommand{\Ain}{{\bf A}_{\rm{in}}}
\newcommand{\beq}{{\bf b}_{\rm{eq}}}
\newcommand{\bin}{{\bf b}_{\rm{in}}}
\newcommand{\bpara}{{\bf b}'}
\newcommand{\Aintilde}{\tilde{{\bf A}}_{\rm{in}}}
\newcommand{\Aindbtilde}{\dbtilde{{\bf A}}_{\rm{in}}}
\newcommand{\setbinding}{\mathcal{X}}

\newcommand{\sgenh}{\mathbf{\hat{s}}^g}
\newcommand{\sloadh}{\mathbf{\hat{s}}^l}
\newcommand{\pflowh}{\mathbf{\hat{\pflow}}}
\newcommand{\angh}{\boldsymbol{\hat{\theta}}}

\newcommand{\dir}{\mathbf{v}}
\newcommand{\EdgeBri}{\mathcal{E}^{\rm bri}}

\newcommand{\GraphT}{\mathcal{G}_{\rm tr}}
\newcommand{\VertexT}{\mathcal{V}_{\rm tr}}

\newcommand{\EdgeT}{\mathcal{E}_{\rm tr}}
\newcommand{\prt}{{\rm par}}
\newcommand{\son}{{\rm son}}

% Sensitivity
\newcommand{\sen}{C}
\newcommand{\wcsen}{C^{\rm wc}}
\newcommand{\ifromj}{{i\leftarrow j}}

% Unicyclic
\newcommand{\GraphCyc}{\mathcal{G}^{\rm O}}
\newcommand{\EdgeCyc}{\mathcal{E}^{\rm O}}
\newcommand{\ec}{e^{\rm O}}
\newcommand{\VertexCyc}{\mathcal{V}^{\rm O}}
\newcommand{\vc}{v^{\rm O}}
\newcommand{\GraphNC}{\mathcal{G}^{\rm nc}}
\newcommand{\EdgeNC}{\mathcal{E}^{\rm nc}}
\newcommand{\VertexNC}{\mathcal{V}^{\rm nc}}
\newcommand{\rt}{\Psi}
\newcommand{\ecut}{e^{\rm cut}}
\newcommand{\mapR}{\Lambda}
\newcommand{\mapRbra}{\Xi}
\newcommand{\ub}[1]{\langle{#1}\rangle}
\newcommand{\myeq}[1]{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny #1}}}{=}}}

% Multiple cycle
\newcommand{\Graphp}{{\mathcal{G}'}}
\newcommand{\Vertexp}{{\mathcal{V}'}}
\newcommand{\Edgep}{{\mathcal{E}'}}
\newcommand{\VertexGp}{\VertexG(\Graphp)}
\newcommand{\VertexLp}{\VertexL(\Graphp)}
\newcommand{\Graphpp}{\mathcal{G}''}
\newcommand{\Vertexpp}{\mathcal{V}''}
\newcommand{\Edgepp}{\mathcal{E}''}
\newcommand{\VertexGpp}{\VertexG(\Graphpp)}
\newcommand{\VertexLpp}{\VertexL(\Graphpp)}
\newcommand{\CMp}{\CM_{\Graphp}}
\newcommand{\CMpp}{\CM_{\Graphpp}}
\newcommand{\avec}{{\bf a}}
\newcommand{\bvec}{{\bf b}}
\newcommand{\xvec}{{\bf x}}
\newcommand{\yvec}{{\bf y}}
\newcommand{\hyvec}{\hat{{\bf y}}}
\newcommand{\zvec}{{\bf z}}
\newcommand{\wvec}{{\bf w}}
\newcommand{\hvec}{{\bf h}}
\newcommand{\col}{{\rm col}}

\newcommand{\GraphCycs}[1]{\mathcal{G}^{{\rm O}_{#1}}}
\newcommand{\VertexCycs}[1]{\mathcal{V}^{{\rm O}_{#1}}}
\newcommand{\EdgeCycs}[1]{\mathcal{E}^{{\rm O}_{#1}}}
\newcommand{\ee}{e^{\diamond}}
\newcommand{\ue}{u^{\diamond}}
\newcommand{\ve}{v^{\diamond}}

\newcommand{\diag}{\textbf{diag}}
\newcommand{\sign}{\textbf{sign}}
\newcommand{\trace}{\textbf{tr}}

%special fonts in computation
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cS}{\mathscr{S}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cD}{\partial}
\newcommand{\DD}{\mathsf{D}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cx}{\mathbf{x}}
\newcommand{\cs}{\mathbf{s}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\cA}{\mathbf{A}}
\newcommand{\cb}{\mathbf{b}}
\newcommand{\cy}{\mathbf{y}}
\newcommand{\ccr}{\mathbf{r}}
\newcommand{\cu}{\mathbf{u}}
\newcommand{\cv}{\mathbf{v}}
\newcommand{\cQMat}{\mathbf{Q}}
\newcommand{\ckappa}{\boldsymbol{\kappa}}
\newcommand{\ctau}{\boldsymbol{tau}}
\newcommand{\cz}{\mathbf{z}}
\newcommand{\cM}{\mathbf{M}}
\newcommand{\cg}{\mathbf{g}}
\newcommand{\ctheta}{\boldsymbol{\Theta}}
\newcommand{\ceta}{\boldsymbol{\eta}}
\newcommand{\cnu}{\boldsymbol{\nu}}
\newcommand{\cW}{\mathbf{W}}
\newcommand{\acC}{\mathbf{C}}

\newcommand{\ja}[1]{{\color{blue}#1}}
\newcommand{\fz}[1]{{\color{brown}#1}}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Optimal Power Flow Operator}{F. Zhou, J. Anderson, and S. H. Low}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{The Optimal Power Flow Operator: Theory and
Computation \thanks{Submitted to the editors DATE.
\funding{This work was funded by NSF grants CCF 1637598, CPS 1739355, and ECCS 1619352, PNNL grant 424858, ARPA-E NODES through grant DE-AR0000699, and through the ARPA-E GRID DATA program.  }}}

% Authors: full names plus addresses.
\author{Fengyu Zhou\thanks{Department of Electrical Engineering, California Institute of Technology, Pasadena, CA 
  (\email{f.zhou@caltech.edu}, \email{slow@caltech.edu}).}
\and James Anderson\thanks{Department of Computing and Mathematical Sciences, California Institute of Technology, Pasadena, CA 
  (\email{james@caltech.edu}).}
\and Steven H. Low\footnotemark[2] \footnotemark[3]}

%\usepackage{amsopn}
%\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> info.tex <==
% Packages and macros go here
\usepackage{lipsum}
\usepackage{epstopdf}
%\usepackage{booktabs} % For formal tables
\usepackage{amsfonts}
\usepackage{mathrsfs} 
\usepackage{amsmath} 
\usepackage{psfrag} 
%\usepackage{multirow} 
%\usepackage{arydshln}
\usepackage{enumerate}
%\usepackage{bbm}
%\usepackage{graphicx}
\usepackage{mathtools}
%\usepackage{color}
%\usepackage{setspace}
%\usepackage{float}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{scalerel}
\usepackage{comment}
\usepackage{gensymb}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{accents}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%\newtheorem{assumption}{Assumption}
%\newcolumntype{Y}{>{\centering\arraybackslash}X}


% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
\newcommand{\dbtilde}[1]{\accentset{\approx}{#1}}


% macros
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\mind}{\min.}
\DeclareMathOperator{\sgn}{sgn}

%\newcommand{\st}{\text{subject to}}
\newcommand{\suchthat}{\text{such that}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Sspace}{\mathbb{S}^+}
\newcommand{\Zset}{\mathbb{Z}}
\newcommand{\T}{\mathsf{T}}
\newcommand{\co}{\mathsf c}
\newcommand{\rank}{{\rm rank}}
\newcommand{\inte}{{\mathrm{int}}}
\newcommand{\clos}{{\mathrm{clos}}}
\newcommand{\base}{{\bf{e}}}
\newcommand{\eye}{\mathbf{I}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\const}{{\rm constant}}
\newcommand{\Ind}{\mathbbm{1}}
\newcommand{\opt}{{\rm opt}}
\newcommand{\fea}{{\rm fea}}
\newcommand{\diff}{\mathrm{d}}

\newcommand{\alphavec}{\boldsymbol{\alpha}}
\newcommand{\betavec}{\boldsymbol{\beta}}

\newcommand{\Graph}{\mathcal{G}}
\newcommand{\Graphnew}{\mathcal{G}_{\rm new}}
\newcommand{\Vertex}{\mathcal{V}}
\newcommand{\VertexG}{\mathcal{V}_{\rm{G}}}
\newcommand{\VertexL}{\mathcal{V}_{\rm{L}}}
\newcommand{\Edge}{\mathcal{E}}
\newcommand{\EdgeI}{\mathcal{E}^{\rm I}}
\newcommand{\EdgeII}{\mathcal{E}^{\rm II}}

\newcommand{\RVertex}{\mathcal{R}}

\newcommand{\nG}{N_{\rm{G}}}
\newcommand{\nL}{N_{\rm{L}}}
\newcommand{\nGL}{N}
\newcommand{\nE}{E}

\newcommand{\CM}{\mathbf{C}}
\newcommand{\B}{\mathbf{B}}

\newcommand{\sgen}{\mathbf{s}^g}
\newcommand{\sgens}{\mathbf{s}_*^g}
\newcommand{\sload}{\mathbf{s}^l}
\newcommand{\sloads}{\mathbf{s}_*^l}
\newcommand{\sloadss}{\mathbf{s}_{**}^l}
\newcommand{\pf}{\mathbf{p}}
\newcommand{\genllim}{\underline{\mathbf{s}}^g}
\newcommand{\genulim}{\overline{\mathbf{s}}^g}

\newcommand{\ang}{\boldsymbol{\theta}}
\newcommand{\angs}{\boldsymbol{\theta}_*}
\newcommand{\f}{{\bf f}}
\newcommand{\fs}{{\bf f}_*}
\newcommand{\fss}{{\bf f}_{**}}
\newcommand{\M}{{\bf M}}
\newcommand{\RelationMat}{{\bf H}}
\newcommand{\subRelationMat}{{\bf H}_1}
\newcommand{\bigMat}{{\bf R}}
\newcommand{\pflow}{{\bf p}}
\newcommand{\pflows}{{\bf p}_*}
\newcommand{\taueq}{\boldsymbol{\tau}}
\newcommand{\mup}{\boldsymbol{\mu}_+}
\newcommand{\mum}{\boldsymbol{\mu}_-}
\newcommand{\mupm}{\boldsymbol{\mu}}
\newcommand{\lambdap}{\boldsymbol{\lambda}_+}
\newcommand{\lambdam}{\boldsymbol{\lambda}_-}
\newcommand{\lambdapm}{\boldsymbol{\lambda}}
\newcommand{\set}{\Omega}
\newcommand{\setbad}{\Omega_{\rm bad}}
\newcommand{\setf}{\Omega_{\f}}
\newcommand{\setsl}{\Omega_{\sload}}
\newcommand{\setsg}{\Omega_{\sgen}}
\newcommand{\setpara}{\Omega_{\para}}
\newcommand{\setall}{\Omega}
\newcommand{\setallr}{\tilde{\Omega}}
\newcommand{\para}{{\boldsymbol{\xi}}}
\newcommand{\paras}{{\boldsymbol{\xi}}_*}
\newcommand{\parass}{{\boldsymbol{\xi}}_{**}}
\newcommand{\setslr}{\widetilde{\Omega}_{\sload}}
\newcommand{\setsgr}{\widetilde{\Omega}_{\sgen}}
\newcommand{\setparar}{\widetilde{\Omega}_{\para}}

\newcommand{\lbold}{\boldsymbol{\lambda}}
\newcommand{\nubold}{\boldsymbol{\nu}}

\newcommand{\setR}{\mathcal{R}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\setT}{\mathcal{T}}
\newcommand{\setQ}{\mathcal{Q}}

\newcommand{\OPF}{\mathcal{OPF}}

\newcommand{\JM}{\mathbf{J}}
\newcommand{\Jwc}{\mathbf{J}^{\rm w}}
\newcommand{\Jsum}{{\boldsymbol \chi}}
\newcommand{\setSgen}{\setS_{\rm G}}
\newcommand{\setSbra}{\setS_{\rm B}}

\newcommand{\Cut}{\mathcal{C}}
\newcommand{\qvec}{{\bf q}}
\newcommand{\tqvec}{\tilde{{\bf q}}}

\newcommand{\dpnoise}{Y}
\newcommand{\mech}{\mathcal{M}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Lap}{\mathscr{L}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\data}{\mathbf{d}}
\newcommand{\dpnoises}{{\bf{Y}}}

\newcommand{\dD}{\mathrm{d}}

% For appendix
\newcommand{\loosegen}{\aleph}
\newcommand{\x}{{\bf x}}
\newcommand{\y}{{\bf y}}
\newcommand{\X}{{\bf X}}
\newcommand{\Y}{{\bf Y}}
\newcommand{\ytilde}{\tilde{\bf y}}
\newcommand{\yreduce}{\underline{\bf y}}
\newcommand{\ytildereduce}{\underline{\tilde{\bf y}}}
\newcommand{\z}{{\bf z}}
\newcommand{\Aeq}{{\bf A}_{\rm{eq}}}
\newcommand{\Ain}{{\bf A}_{\rm{in}}}
\newcommand{\beq}{{\bf b}_{\rm{eq}}}
\newcommand{\bin}{{\bf b}_{\rm{in}}}
\newcommand{\bpara}{{\bf b}'}
\newcommand{\Aintilde}{\tilde{{\bf A}}_{\rm{in}}}
\newcommand{\Aindbtilde}{\dbtilde{{\bf A}}_{\rm{in}}}
\newcommand{\setbinding}{\mathcal{X}}

\newcommand{\sgenh}{\mathbf{\hat{s}}^g}
\newcommand{\sloadh}{\mathbf{\hat{s}}^l}
\newcommand{\pflowh}{\mathbf{\hat{\pflow}}}
\newcommand{\angh}{\boldsymbol{\hat{\theta}}}

\newcommand{\dir}{\mathbf{v}}
\newcommand{\EdgeBri}{\mathcal{E}^{\rm bri}}

\newcommand{\GraphT}{\mathcal{G}_{\rm tr}}
\newcommand{\VertexT}{\mathcal{V}_{\rm tr}}

\newcommand{\EdgeT}{\mathcal{E}_{\rm tr}}
\newcommand{\prt}{{\rm par}}
\newcommand{\son}{{\rm son}}

% Sensitivity
\newcommand{\sen}{C}
\newcommand{\wcsen}{C^{\rm wc}}
\newcommand{\ifromj}{{i\leftarrow j}}

% Unicyclic
\newcommand{\GraphCyc}{\mathcal{G}^{\rm O}}
\newcommand{\EdgeCyc}{\mathcal{E}^{\rm O}}
\newcommand{\ec}{e^{\rm O}}
\newcommand{\VertexCyc}{\mathcal{V}^{\rm O}}
\newcommand{\vc}{v^{\rm O}}
\newcommand{\GraphNC}{\mathcal{G}^{\rm nc}}
\newcommand{\EdgeNC}{\mathcal{E}^{\rm nc}}
\newcommand{\VertexNC}{\mathcal{V}^{\rm nc}}
\newcommand{\rt}{\Psi}
\newcommand{\ecut}{e^{\rm cut}}
\newcommand{\mapR}{\Lambda}
\newcommand{\mapRbra}{\Xi}
\newcommand{\ub}[1]{\langle{#1}\rangle}
\newcommand{\myeq}[1]{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny #1}}}{=}}}

% Multiple cycle
\newcommand{\Graphp}{{\mathcal{G}'}}
\newcommand{\Vertexp}{{\mathcal{V}'}}
\newcommand{\Edgep}{{\mathcal{E}'}}
\newcommand{\VertexGp}{\VertexG(\Graphp)}
\newcommand{\VertexLp}{\VertexL(\Graphp)}
\newcommand{\Graphpp}{\mathcal{G}''}
\newcommand{\Vertexpp}{\mathcal{V}''}
\newcommand{\Edgepp}{\mathcal{E}''}
\newcommand{\VertexGpp}{\VertexG(\Graphpp)}
\newcommand{\VertexLpp}{\VertexL(\Graphpp)}
\newcommand{\CMp}{\CM_{\Graphp}}
\newcommand{\CMpp}{\CM_{\Graphpp}}
\newcommand{\avec}{{\bf a}}
\newcommand{\bvec}{{\bf b}}
\newcommand{\xvec}{{\bf x}}
\newcommand{\yvec}{{\bf y}}
\newcommand{\hyvec}{\hat{{\bf y}}}
\newcommand{\zvec}{{\bf z}}
\newcommand{\wvec}{{\bf w}}
\newcommand{\hvec}{{\bf h}}
\newcommand{\col}{{\rm col}}

\newcommand{\GraphCycs}[1]{\mathcal{G}^{{\rm O}_{#1}}}
\newcommand{\VertexCycs}[1]{\mathcal{V}^{{\rm O}_{#1}}}
\newcommand{\EdgeCycs}[1]{\mathcal{E}^{{\rm O}_{#1}}}
\newcommand{\ee}{e^{\diamond}}
\newcommand{\ue}{u^{\diamond}}
\newcommand{\ve}{v^{\diamond}}

\newcommand{\diag}{\textbf{diag}}
\newcommand{\sign}{\textbf{sign}}
\newcommand{\trace}{\textbf{tr}}

%special fonts in computation
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cS}{\mathscr{S}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cD}{\partial}
\newcommand{\DD}{\mathsf{D}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cx}{\mathbf{x}}
\newcommand{\cs}{\mathbf{s}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\cA}{\mathbf{A}}
\newcommand{\cb}{\mathbf{b}}
\newcommand{\cy}{\mathbf{y}}
\newcommand{\ccr}{\mathbf{r}}
\newcommand{\cu}{\mathbf{u}}
\newcommand{\cv}{\mathbf{v}}
\newcommand{\cQMat}{\mathbf{Q}}
\newcommand{\ckappa}{\boldsymbol{\kappa}}
\newcommand{\ctau}{\boldsymbol{tau}}
\newcommand{\cz}{\mathbf{z}}
\newcommand{\cM}{\mathbf{M}}
\newcommand{\cg}{\mathbf{g}}
\newcommand{\ctheta}{\boldsymbol{\Theta}}
\newcommand{\ceta}{\boldsymbol{\eta}}
\newcommand{\cnu}{\boldsymbol{\nu}}
\newcommand{\cW}{\mathbf{W}}
\newcommand{\acC}{\mathbf{C}}

\newcommand{\ja}[1]{{\color{blue}#1}}
\newcommand{\fz}[1]{{\color{brown}#1}}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Optimal Power Flow Operator}{F. Zhou, J. Anderson, and S. H. Low}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{The Optimal Power Flow Operator: Theory and
Computation \thanks{Submitted to the editors DATE.
\funding{This work was funded by NSF grants CCF 1637598, CPS 1739355, and ECCS 1619352, PNNL grant 424858, ARPA-E NODES through grant DE-AR0000699, and through the ARPA-E GRID DATA program.  }}}

% Authors: full names plus addresses.
\author{Fengyu Zhou\thanks{Department of Electrical Engineering, California Institute of Technology, Pasadena, CA 
  (\email{f.zhou@caltech.edu}, \email{slow@caltech.edu}).}
\and James Anderson\thanks{Department of Computing and Mathematical Sciences, California Institute of Technology, Pasadena, CA 
  (\email{james@caltech.edu}).}
\and Steven H. Low\footnotemark[2] \footnotemark[3]}

%\usepackage{amsopn}
%\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

